Distributionally Robust Optimal and Safe Control of Stochastic Systems via Kernel Conditional Mean Embedding

We present a novel distributionally robust framework for dynamic programming that uses kernel methods to design feedback control policies. Specifically, we leverage kernel mean embedding to map the transition probabilities governing the state evolution into an associated repreducing kernel Hilbert space. Our key idea lies in combining conditional mean embedding with the maximum mean discrepancy distance to construct an ambiguity set, and then design a robust control policy using techniques from distributionally robust optimization. The main theoretical contribution of this paper is to leverage functional analytic tools to prove that optimal policies for this infinite-dimensional min-max problem are Markovian and deterministic. Additionally, we discuss approximation schemes based on state and input discretization to make the approach computationally tractable. To validate the theoretical findings, we conduct an experiment on safe control for thermostatically controlled loads (TCL).

==> Sections/legacy.tex <==
%%%% OLD MATERIAL %%%%%%

\ashish{Add general theory of DR-Stochastic Control, minmax interchange, markovian policy, etc}

\ignore{\licio{This is just a suggestion. I would start formulating the problem using the general framework that will be presented in the previous section and then specialise it to both the safety and reach-avoid case.

Let's imagine that we can come up with general theorem that guarantee existence and uniqueness of Markov policies of DR dynamic programming using the stochastic model that I will describe. Then rather than following the structure of previous papers in the literature (such as Yang, etc), we could employ our own tools to show well-posedness of our mathematical formulation (at least for the journal version; the conference version we could adopt a shortcut citing existing results). 

In the conference version, I was planning to connect directly to literature in functional analysis, etc, rather than citing directly the papers in the control community (of course, their result will be acknowledged at some other stages of our paper).

Below is the structure that I was thinking for this part of the paper:

\begin{itemize}
    \item Introduce the dynamical programming iteration considering ambiguity sets. At this stage, I would only mention general properties of the value function (upper semi-continuity, measurability, compactness of the ambiguity sets, etc) and present the formulation using ambiguity sets. At the end of this description, we should be able to have a DP iteration that will look like
    \begin{equation}
        v_{k}(x) = \inf_{u \in \mathcal{U}} \sup_{T(\cdot|x,u) \in \mathcal{A}} \int_{\mathbb{R}^n} v_{k+1}(\xi) T(d\xi|x,u),
        \label{eq:DPFormulation}
    \end{equation}
    and we should be able to show that this problem is well-defined by tapping into the results from functional analysis and the description of discrete-time stochastic models that I will describe in the beginning of the paper.
    
    \item We could then specialise \eqref{eq:DPFormulation} to the safety and reach-avoid problem for all the ambiguity sets that were introduced in previous section of the paper. And, in doing so, we show that each of the regularity conditions are satisfied.
    
    \item Once this is done, we turn into methods that are used to approximate the solution of \eqref{eq:DPFormulation} using samples. Here are that we should mention in this part:
    
    \begin{itemize}
        \item Duality for the approximation of the resulting semi-infinite optimisation problems.
        \item Statistical complexities whenever one is able to provide.
    \end{itemize}
    
    
    \end{itemize}


Please do let me know what you think about this Ashish. Happy to hear your thoughts.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $x_k \in \Rb^\dimState$ and $u_k \in \mathcal{U} \subset \Rb^\dimControl$ denote the state and control input of a discrete-time stochastic dynamical system with $\mathcal{U}$ being a closed subset of admissible inputs. The state evolution is governed by a stochastic kernel $T: \Rb^\dimState \times \Rb^\dimControl \mapsto \spaceOfMeas{\dimState}$ where $\spaceOfMeas{\dimState}$ denotes the set of probability measures defined on $\Rb^\dimState$. We are interested in the paths generated by the discrete-time stochastic process
\begin{equation}
x_{k+1} \sim T(\cdot|x_k,u_k), \quad u_k \in \mathcal{U}, \quad x_0 = \bar{x},
\label{eq:DT_stochasticSystem}    
\end{equation}
where the next state is sampled from the probability measure defined by the pair $(x_k,u_k)$ through the underlying stochastic kernel. This description of discrete-time stochastic systems has been inspired by the papers \cite{Wit:73,Wit:88} and will prove to be adequate to our purposes.

Notice that the description \eqref{eq:DT_stochasticSystem} is general enough to encompass well-known classes of discrete-time stochastic systems. For instance, the class of linear systems 
\[
x_{k+1} = A x_k + B u_k + \noise_k, \quad u_k \in \mathcal{U}, \quad \noise_k \sim \normalDist{0}{\Sigma},
\]
with zero-mean additive Gaussian noise can be seen in the context presented in \eqref{eq:DT_stochasticSystem} where for any Borel subset $V \subset \Rb^\dimState$ we have
\[
T(V|x_k,u_k) = \frac{1}{(2\pi)^{\frac{n}{2}}} \frac{1}{\mathrm{\Sigma}^{\frac{1}{2}}} \int_{V} e^{-\frac{1}{2}(\xi-\bar{x}_{k+1})^\top \Sigma^{-1} (\xi-\bar{x}_{k+1})} d\xi,
\]
where $\bar{x}_{k+1}:=Ax_k+Bu_k$, i.e., for each pair $(x_k,u_k)$ the stochastic kernel is a multivariate Gaussian distribution with mean $\bar{x}_{k+1}$ and covariance $\Sigma$. We can also model the class of discrete-time hybrid systems \cite{APLS:08,APLP:10} using the formulation of equation \eqref{eq:DT_stochasticSystem} by merging both the discrete and continuous kernels. Details are omitted for brevity.

We now introduce the formal construction of the measure in the space of sequences induced by the stochastic kernel that generates the trajectories of system \eqref{eq:DT_stochasticSystem}. To this end, consider the space of finite sequences
\begin{equation}
    \spaceFiniteSeq{N} = \{ (x_1,\ldots,x_N): x_i \in \Rb^\dimState \},
    \label{eq:SpaceofFiniteSequences}
\end{equation}
and denote a generic element in \spaceFiniteSeq{N} by $\mathbf{x}_N$. Let $V_1, \ldots, V_N$ be a collection of closed subsets of $\Rb^\dimState$ and  $\controlPolicy: \Rb^\dimState \mapsto \Rb^\dimControl$ be a given control policy, then the kernel $T$ induces a probability measure on the subset $\prod_{i = 1}^N V_i$ as 
\begin{align}
    & \probSeq_{\controlPolicy,\bar{x}}^N \left\{ \mathbf{x}_N \in \prod_{i = 1}^N V_i \right\} = \int_{V_1} \ldots \int_{V_N} \nonumber
    \\ & \qquad T(dx_N| x_{N-1},\controlPolicy(x_{N-1})) \ldots T(dx_1| \bar{x},\controlPolicy(\bar{x})).
    \label{eq:ProbFiniteSequence}
\end{align}
Since the collection of measures $(\probSeq_{\pi,\bar{x}}^N)_{N \in \mathbb{N}}$ satisfies the conditions of the Kolmogorov extension theorem, it can be uniquely extended to the whole space of sequences.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Distributionally Robust Safety Specification}



In safety-critical applications, the trajectory of \eqref{eq:DT_stochasticSystem} leaving a (safe) region of the state space may have catastrophic consequences. We consider the distributionally robust version of the problem where the stochastic transition kernel is not known, rather it belongs to a family of probability distributions or {\it ambiguity set} that contain the true distribution with high probability. Motivated by this fact, in this paper we would like to design a control law that is robust with respect to the mechanism generating the trajectory and that guarantees a lower bound on the probability that the trajectories of \eqref{eq:DT_stochasticSystem} remain in a given safe set $S \subset \Rb^n$ for a finite horizon of length $T$.

We first introduce the distributionally robust dynamic programming operator $\mathcal{T}$ for a measurable function $v$ on $\mathbb{R}^n$ as
\begin{equation}
(\mathcal{T}v)(x) = \inf_{u \in \mathcal{U}} \sup_{T(\cdot|x,u) \in \mathcal{A}} \int_{\mathbb{R}^n} v(\xi) T(d\xi|x,u).
\label{eq:dp_main}        
\end{equation}

Under suitable technical conditions, the dynamic programming iterations for the discrete-time stochastic control problem can be stated recursively as 
$$ v_N(x) = c(x), v_{k}(x) = (\mathcal{T}v_{k+1})(x), 0 \leq k \leq N-1.$$
One can also show that distributionally robust safety and reach-avoid formulations can be stated in the above manner. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reformulation of the Bellman Operator}

\ashish{You have written the DP iteration in \eqref{eq:DPFormulation} as
    \begin{equation*}
        v_{k}(x) = \inf_{u \in \mathcal{U}} \sup_{T(\cdot|x,u) \in \mathcal{A}} \int_{\mathbb{R}^n} v_{k+1}(\xi) T(d\xi|x,u).
    \end{equation*}
There are two possibilities here: (i) ambiguity set $\mathcal{A}$ depends on control input $u$ and $x$ and (ii) $\mathcal{A}$ is independent of $x$ and $u$. Most prior work, including the ones by Insoon consider case (ii). Case (i) would result in a two stage optimization problem with decision-dependent ambiguity set which is in general a more difficult problem class. Something to keep in mind and discuss.

In the following text, I proceed by presenting the reformulation of \eqref{eq:dp_op_safety}. 
}

Recall that the Bellman equation for the finite-horizon distributionally robust stochastic control problem is given by
\begin{equation}\label{eq:bellman_minmax_gen}
        v_t(x) = \max_{u \in U(x)} \inf_{\gamma \in \Gamma_t} \int_{\Wb_t} v_{t+1}(f(x,u,\noise_t)) d\gamma(\noise_t), \qquad t \in \{0,1,\ldots,T-1\},
\end{equation}
where $\Wb_t$ is the support of $\noise_t$. We now present finite dimensional reformulations of the above problem under different ambiguity sets. 


\subsection{Reformulation under Moment-based ambiguity sets}

\subsection{Reformulation under Wasserstein ambiguity sets}

Consider the Bellman equation \eqref{eq:bellman_minmax_gen} under Wasserstein ambiguity set, i.e., with $\Gamma_t = \MM^\theta_N = \{\mu \in \PP_p(\Xi)| W_p(\mu,\Pbhat_N) \leq \theta\}$ defined in \eqref{eq:wasserstein-set} with the empirical distribution being $\Pbhat_N := \frac{1}{N}\sum^N_{i=1} \delta_{\noise_i}$ constructed from observed samples. We have the following reformulation of \eqref{eq:bellman_minmax_gen} as a consequence of Theorem \ref{theorem:gao_duality}. 

\begin{proposition}\label{prop:wasserstein_bellman}
Suppose $v_{t+1}$ is lower semi-continuous and $\Wb_t$ is compact. Then, \eqref{eq:bellman_minmax_gen} can be stated as
\begin{align}
    v_t(x) = & \sup_{u, \lambda, s} \quad \lambda \theta^p + \frac{1}{N} \sum^N_{i=1} s_i, \nonumber 
    \\ & \text{s.t.} \quad v_{t+1}(f(x,u,\noise)) - \lambda d^p(\noise,\noise_i) \leq s_i, \qquad \forall \noise \in \Wb_t, \label{eq:bellman_dual_wasserstein} 
    \\ & \qquad u \in U(x), \quad \lambda \geq 0, \quad s \in \Rb^N. \nonumber 
\end{align}
\end{proposition}

Note that in Theorem \ref{theorem:gao_duality}, the supremum was with respect to the ambiguity set while the function $H$ was required to be upper semi-continuous. In the Bellman equation, we have the infimum with respect to the ambiguity set, and as a result, the value function $v_{t+1}$ is required to be lower semi-continuous. Note further than unless $\Wb_t$ has finite cardinality, \eqref{eq:bellman_dual_wasserstein} is a semi-infinite program. 

\ashish{Need to be careful with semi-continuity. In the alternative formulation \eqref{eq:DPFormulation} you have given, what would the distance $d^p$ measure? Would it be $v_{t+1}(x_+) - d^p(x_{+},\hat{x}_{+,i}) \leq s_i, \qquad \forall x_{+} \in \mathcal{X}$?}

\subsection{Reformulation under Kernel-based ambiguity sets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage 

We now present the reformulation of \eqref{eq:bellman_minmax_gen} under MMD ambiguity sets \eqref{eq:mmd-ambiguity-set} induced by observed samples as a consequence of Theorem \ref{theorem:kernel_dro_duality}. 

\begin{proposition}\label{prop:rkhs_bellman}
Suppose $v_{t+1}$ is lower semi-continuous, $\Wb_t$ is compact and $\Gamma_t = \mathtt{MMD}^\theta_N$. Then, \eqref{eq:bellman_minmax_gen} can be stated as
\begin{align}
    v_t(x) = & \sup_{u, f_0, f} \quad f_0 + \theta ||f||_\HH + \frac{1}{N} \sum^N_{i=1} f(\noise_i), \nonumber 
    \\ & \text{s.t.} \quad v_{t+1}(f(x,u,\noise)) \leq f_0 + f(\noise), \qquad \forall \noise \in \Wb_t, \label{eq:bellman_dual_kernel} 
    \\ & \qquad u \in U(x), \quad f \in \HH, \quad f_0 \in \Rb. \nonumber 
\end{align}
\end{proposition}


\newpage 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Reformulation under Kernel Ambiguity}

We now have all the ingredients to tackle equation \eqref{eq:dp_main} in the context of kernel mean embeddings. Let us rewrite \eqref{eq:dp_main} using a slightly different notation:
\begin{equation}
    g(x) = \inf_{u \in \mathcal{U}} \sup_{\mathbb{P} \in \mathcal{A}} \int_{\mathbb{R}^n} v(\xi) d \mathbb{P}(\xi)
    \label{eq:DPFormulation2},
\end{equation}
where we substitute $v_k$ by $g$, $v_{k+1}$ by $v$, and $T(\cdot|x,u)$ by $\mathbb{P}$. Our goal is to compute the function $g$ given in \eqref{eq:DPFormulation2} when $\mathcal{A}$ is constructed using a kernel associated with the Euclidean space.

Let $x \in \mathbb{R}^n, u \in \Rb^p$ be fixed and consider the inner problem in \eqref{eq:DPFormulation2} when the ambiguity set $\mathcal{A}$ is given by
\[
\mathcal{A} = \{ \mathbb{Q} \in \mathcal{P}(\mathbb{R}^n): \int_{\mathbb{R}^n} k(\cdot,\xi) d \mathbb{Q}(\xi) \in \mathcal{C}  \},
\]
where $\mathcal{C}$ is a subset of the RKHS $\mathcal{H}$. In other words, $\mathcal{A}$ contains all distributions whose kernel mean embeddings belong to a subset of the Hilbert space, e.g., the MMD ambiguity set defined in \eqref{eq:mmd-ambiguity-set}. 

Using the definition of the kernel mean embedding mapping given in \eqref{eq:KernelMeanEmbedding}, one may notice that the ambiguity can be written as $\mathcal{A} = \Psi^{-1}(\mathcal{C})$, i.e., it is the inverse image of the set $\mathcal{C}$ under the mapping $\Psi$. With this notation and using the dual pairing definition, we may write the inner optimization problem in \eqref{eq:DPFormulation2} as
\begin{align*}
\sup_{\mathbb{P} \in \mathcal{A}} \inner{v}{\mathbb{P}} & = \sup_{\mathbb{P} \in \Psi^{-1}(\mathcal{C})} \inner{v}{\mathbb{P}} = \sup_{\Psi(\mathbb{P}) \in \mathcal{C}} \inner{v}{\mathbb{P}}.
\end{align*}

A consequence of the reproducing property of RKHS is
\begin{align*}
\innerRKHS{v}{\Psi(\mathbb{P})} & = \innerRKHS{v}{\int_{\mathbb{R}^n} k(\cdot,\xi') d\mathbb{P}(\xi')}
\\ & = \int_{\mathbb{R}^n} \innerRKHS{v}{k(\cdot,\xi')} d\mathbb{P}(\xi')
\\ & = \int_{\mathbb{R}^n} v(\xi') d\mathbb{P}(\xi') = \inner{v}{\mathbb{P}},
\end{align*}
for all $\mathbb{P} \in \mathcal{P}(\mathbb{R}^n)$ and for all $v \in \mathcal{H}$, i.e., the expectation of a function $v$ can be stated equivalently as the inner product of the function with the kernel mean embeddeding of the distribution \cite{smola2007hilbert}. Hence, we can write the inner optimization problem in \eqref{eq:DPFormulation2} as
\[
\sup_{\Psi(\mathbb{P}) \in \mathcal{C}} \inner{v}{\mathbb{P}} = \sup_{\Psi(\mathbb{P}) \in \mathcal{C}} \innerRKHS{v}{\Psi(\mathbb{P})} = \sigma_{\mathcal{C}} (v),
\]
where $\sigma_{\mathcal{C}}$ is the support function of the set $\mathcal{C}$.  

We now focus on the support function $\sigma_{\mathcal{C}}$ for the class of MMD ambiguity sets constructed from samples. Suppose the empirical distribution $\widehat{\Pb}_N := \sum^N_{i=1} \alpha_i \delta_{\omega_i}$ with $\sum_{i = 1}^N \alpha_i = 1, \alpha_i \geq 0, i = 1, \ldots, N$, where $x_1, \ldots, x_N$ are samples from the set $\mathbb{R}^n$. The kernel mean embeddeding $\Psi(\widehat{\Pb}_N)(x) = \sum_{i = 1}^N \alpha_i k(x,x_i)$. Consequently, the set $\mathcal{C}^\epsilon$ is given by
\[
\mathcal{C}^\epsilon = \{ h \in \mathcal{H}: \normRKHS{h - \Psi(\widehat{\Pb}_N)} \leq \epsilon \},
\]
for some $\epsilon > 0$. 


%However, notice that the following relation holds:
%\begin{align*}
%\innerRKHS{v}{\Psi(\mathbb{P})} & = \int_{\mathbb{R}^n} v(\xi) \int_{\mathbb{R}^n} k(\xi,\xi') d\mathbb{P}(\xi') d\mathbb{P}(\xi) 
%\\ & = \int_{\mathbb{R}^n} \underbrace{\int_{\mathbb{R}^n} v(\xi) k(\xi,\xi') d \mathbb{P}(\xi)}_{\innerRKHS{v}{k(\cdot,\xi')} = v(\xi')} d \mathbb{P}(\xi') = \inner{v}{\mathbb{P}},
%\end{align*}
%that is the dual pairing $\inner{v}{\mathbb{P}}$ is equal to the inner product $\innerRKHS{v}{\Psi(\mathbb{P})}$ for all $\mathbb{P} \in \mathcal{P}(\mathbb{R}^n)$ and for all $v \in \mathcal{H}$. 

\sloppy
Let $H_t$ denote the set of histories upto time $t$ with elements of the form $h_t = (x_0, u_0, \noise_0, \ldots, x_{t-1}, u_{t-1}, \noise_{t-1}, x_t)$. The set of admissible control policies is given by $\Pi = \{(\pi_0,\pi_1,\ldots,\pi_{T-1})|\pi_t(U(x_t)|h_t) = 1, \forall h_t \in H_t\}$ where $U(x_t)$ is the set of control inputs that are admissible at state $x_t$. 

Let $\gamma_t$ denote the distribution of $\noise_t$. Past works such as \cite{yang2018dynamic,ding2013stochastic} assume that $\gamma_t$ depends on the past trajectory and ambiguity sets, possibly in a Markovian manner, and chosen by an adversarial agent from a set of admissible disturbance distributions. However, for brevity of notation, we omit such dependencies, and simply denote the ambiguity set of disturbance distributions by $\Gamma := \Pi^{T-1}_{t = 0} \Gamma_t$ with $\gamma_t \in \Gamma_t$. A sequence of disturbance distributions is denoted by $\gamma = (\gamma_0,\gamma_1,\ldots,\gamma_{T-1})$. 

There are two main ingredients that are required to solve the above problem. 
\begin{enumerate}
    \item First we need to show that there exists a non-randomized Markov policy that maximizes the worst case safety probability. The main step is to show that upper semi-continuity of the value function is preserved through the dynamic programming operator. Leveraging the seminal results in \cite{gonzalez2002minimax}, \cite{yang2018dynamic,yang2020wasserstein} showed that the following assumptions are sufficient to guarantee that upper semi-continuity is preserved under moment and Wasserstein ambiguity sets, respectively. 
    \begin{assumption}
    The following conditions hold.
    \begin{enumerate}
        \item For any bounded continuous function $g: \Rb^n \to \Rb$, the function $\hat{g}(x,u,\gamma) := \int_{\Rb^r} g(f(x,u,\noise)) d\gamma(\noise)$ is continuous in $(x,u,\gamma)$ for each $\gamma \in \Gamma$.
        \item The set $U(x)$ is compact for each $x \in \Rb^n$. Furthermore, the set-valued mapping $x \mapsto U(x)$ is upper semi-continuous.
        \item The safety set $\safeSet$ is compact. 
    \end{enumerate}
    \end{assumption}
    \item When the existence of an optimal non-randomized Markovian policy is established, the next challenge is to obtain a tractable solution of the Bellman equation which can now be stated as
    \begin{equation}\label{eq:bellman_minmax}
        v_t(x) = \max_{u \in U(x)} \inf_{\gamma \in \Gamma_t} \mathbf{1}_\safeSet(x) \int_{\Rb^r} v_{t+1}(f(x,u,\noise)) d\gamma(\noise), 
    \end{equation}
    for $t \in \{0,1,\ldots,T-1\}$. The inner problem of the above Bellman equation is infinite dimensional as it requires finding an extremal distribution from the ambiguity set. One needs to reformulate the inner problem using suitable duality results as appropriate for the underlying ambiguity set.
\end{enumerate}
